Dialects for CoAP-like Messaging Protocols

Messaging protocols for resource limited systems such as distributed IoT systems are often vulnerable to attacks due to security choices made to conserve resources such as time, memory, or bandwidth. For example, use of secure layers such as DTLS are resource expensive and can sometimes cause service disruption. Protocol dialects are intended as a light weight, modular mechanism to provide selected security guarantees, such as authentication. In this report we study the CoAP messaging protocol and define two attack models formalizing different vulnerabilities. We propose a generic dialect for CoAP messaging. The CoAP protocol, dialect, and attack models are formalized in the rewriting logic system Maude. A number of case studies are reported illustrating vulnerabilities and effects of applying the dialect. We also prove (stuttering) bisimulations between CoAP messaging applications and dialected versions, thus ensuring that dialecting preserves LTL properties (without Next) of CoAP applications. To support search for attacks in complex messaging situations we specify a simple application layer to drive the CoAP messaging and generalize the attack model to support a form of symbolic search for attacks. Two case studies are presented to illustrate the more general attack search.

==> coap-attacks-table.tex <==
\begin{table}[ht]
\begin{center}
  \begin{tabular}{|l|c|r|r|} %% {p{3.3cm}p{2.5cm}p{5.5cm}}
  \hline
  \textbf{Scenario}\quad &\textbf{~D?~}& \textbf{success} & \quad\textbf{fail} \\
 \hline
   (Fig 1)         & C & 2/7 & NS \\
                      & D & 2/9 & NS \\
 \hline
   (Fig 2)          & C & 3/528 &  NS \\
                       & D & 8/2417 & NS \\
 \hline
  (Fig 3)           & C & 4/330 & 4/326 \\
                       & D & 4/499 & 4/496 \\
 \hline
  (Fig 4)         & C & 8/260  & 45/2586 \\
                    & D & 16/10167 & 86/10076 \\
 \hline
  (Fig 5)           & C & NS &  \\
                     & D & NS &  \\
 \hline
  (Fig 5x)         & C & 4/330 &  \\
                     & D & 4/499 & \\
 \hline
  (Fig 6)            & C & NS & \\
                      & D & NS &     \\
 \hline  
  (Fig 6x)           &C & 18/2742 & \\
                      & D & 18/4675df &   \\
 \hline
  (vi) Fig 7          & C & NS &    \\
                      & D & NS &     \\
 \hline
  (viim) Fig 7mod      &C  & 4/33 & \\
                       & D & NS  &     \\
 \hline
  \end{tabular}
\end{center}
\caption{Reachability results for CoAP vulnerability scenarios with and without dialect wrapping.}
\label{tb:coap-attacks}
\end{table}


==> exe-props-old.tex <==
\section{Characterization of reachable CoAP system configuration

The following are basic properties of
configurations reachable from an initial
configuration useful in reasoning about higher
level properties.

\omitthis{
CoAP system configurations \texttt{sysC} have the form~\footnote{We assume $k>=2$, no point in talking to yourself}
 \begin{small}
 \begin{verbatim}
   { [eid-j | devatts-j ] | 0 <= j < k 
     net(dmsgs0,dmsgs1)
     ["eve" | kb(dmsgs) caps(caps)]
     } 
 \end{verbatim}
 \end{small}

\noindent
The attributes \texttt{devatts-j} have the form
\begin{small}
\begin{verbatim}
    sendReqs(amsgl:AMsgL) rsrcs(rbnds:RMap)   
    w4Ack(dmsgs:DMsgS) w4Rsp(msgs:MsgS) 
    rspSntD(dmsgs1:DMsgS) rspRcd(msgs1:DMsgS)
    ctr(n) config(coap-config)
\end{verbatim}
\end{small}
\noindent 
where the constant \texttt{coap-config} sets the
global configuration parameters such as the time to
wait for a message acknowledgement before
resending, and the maximal number of retransmits.
\footnote{Note the no attacker case is represented by caps = capsd = mtC.}

}

\omitthis{
Dialected CoAP system configurations, \texttt{dsysC}, have the form
 \begin{small}
 \begin{verbatim}
   { [eid-j | conf([eid-j | devatts'-j] 
                   net(dmsgsO-j,dmsgsI-j) --- local net
                   )
              ddevatts-j ]   
     | 0 <= j < k 
     net(ddmsgs0,ddmsgs1)  --- global net
     [eve | kb(ddmsgs) caps(capsd)]
     } 
 \end{verbatim}
 \end{small}

The dialect attributes \texttt{ddevatts-j} of
\texttt{eid-j} include a triple of attributes of
the form

\begin{small}
\begin{verbatim}
seedFr(eid-k,seedF(eid-k)),seedTo(eid-k,seedT(eid-k)),ixCtr(eid-k,0)    
\end{verbatim}     
\end{small}
\noindent
for  each $\mathtt{k} \neq \mathtt{j}$. 
They also include attributes
\texttt{randSize(128)} and
\texttt{used(ubnds:UMap)} where \texttt{ubnds:UMap}
is a map from endpoint ids to the set of lingo indices used in dialecting messages from that
endpoint.
}

We define initial system configurations (basic CoAP
and dialected versions) and restrict attention to
configurations reachable from inital configurations
by application of the rewrite rules.

\begin{definition}[Initial CoAP configuration]
  \label{defn:sysI}
An initial CoAP system configuration \texttt{sysI} has 
an empty network, empty wait4 and response attributes.  More precisely \texttt{sysI}
contains one
network configuration element of the form
\texttt{net(mtDM,mtDM)} and a finite number of
endpoint agents of the form 
\begin{small}
\begin{verbatim}
    [eid | sendReqs(amsgl:AMsgL) rsrcs(rbnds:RMap)  
           initDevAttrs]
\end{verbatim}
\end{small}
\noindent
where \texttt{initDevAttrs} is the attribute set
\begin{small}
\begin{verbatim}
    w4Ack(mtDM) w4Rsp(mtM)rspSntD(mtDM) rspRcd(mtM)
    ctr(0) config(coap-config)
\end{verbatim}
\end{small}

An initial system
configuration with attacker also has an attack
agent (which we omit if \texttt{caps:Caps} is empty).
\begin{small}
\begin{verbatim}
[ "eve" | kb(dmsgs) caps(caps:Caps)]
\end{verbatim}
\end{small}
\end{definition}

We define the dialecting transform \texttt{D(sysI)} that wraps an initial CoAP system configurate as above to become an initial dialected
configuration, \texttt{dsysI}.

\begin{definition}[CoAP Dialect Transformation]
  \label{defn:d-xform}
Let \texttt{sysI} be as above and
let \texttt{eids} be the set of endpoint identifiers
$\{\mathtt{eid-j} |\mathtt{ 0} \leq \mathtt{j} < \mathtt{k}\}$ of  \texttt{sysI}.
Then \texttt{D(sysI)} is a dialected system configuration of the form given above with
the same set of endpoint identifiers and where
\begin{itemize}
\item
 $\mathtt{devatts'-j} =  \mathtt{devatts-j}$ 
 for $\mathtt{0} \leq \mathtt{j} <  \mathtt{k}$
\item
all (local and global) net elements are empty
(\texttt{mtDM})
\item
  $\mathtt{caps} = \mathtt{capsd}$
\item
\texttt{ddevats-j} is constructed as shown for
the generic dialected system above where
the used attribute is \texttt{used(mtU)}.
\end{itemize}
\end{definition}
\noindent
Note: In the test scenarios the seed constructors
for eid-j are defined as
$\mathtt{seedF(eid-k)} =\mathtt{"xxxx"+eid-j+eid-k}$ 
 and
 $\mathtt{seedT(eid-k)} = \mathtt{"xxxx"+eid-k+eid-j}$.
At the level of abstract of the Maude model
all that is required is that the seeds be
distinct since no operations are provided
for the attacker to compute with them.

Note that  the use of \texttt{eids} in  the dialect wrapper function
assumes all pairs of endpoints communicate.
This could be refined by computing a list
of communicating pairs from the initial \texttt{sendReqs} list for each 
endpoint of \texttt{sysI}.



\begin{definition}[Initial dialected CoAP configuration]\label{defn:dsysI}
An initial dialected CoAP system, \texttt{dsysI}, is the
result of transforming an initial CoAP system 
\texttt{sysI}
($\mathtt{dsysI} = \mathtt{D}(\mathtt{sysI},\mathtt{eids})$) where
\texttt{eids} is the set of endpoint identifiers of
\texttt{sysI}.
\end{definition}


The minimum time to elapse function, \texttt{mte},
returns a value that is either \texttt{0},
\texttt{nz : NzNat} or \texttt{infty}. The
following propositions give essential properties of
reachable CoAP and dialected CoAP system
configurations according to the \texttt{mte} value.

\begin{proposition}[Mte based characterization of reachable CoAP configurations]\label{prop:mte-coap}
Let \texttt{sysI}  be an initial configuration 
and let  \texttt{sysC} be a CoAP system configuration
reachable from \texttt{sysI}.   Then one of the following
holds.
\begin{itemize}
\item[1.] \texttt{mte(sysC) = nz:NzNat}.
In this case the tick rule is enabled (and no other
rule is enabled (except possibly \texttt{net} which
commutes with and is independent of \texttt{tick}).
Further more
\begin{itemize}
\item  
 for all \texttt{msg @ d} in the network,  $\mathtt{d} > 0$ (ow \texttt{mte} is 0). 
\item  
for all \texttt{msg @ d} in some \texttt{w4Ack} attribute $\mathtt{d} > 0$  (ow \texttt{mte} is 0). 
\item  
if the \texttt{sendReq} attribute of some endpoint is not empty (\texttt{nilAM}) then either there are more than the \texttt{w4Ack} limit of requests
waiting for acknowledgement
(and hence rule \texttt{devsnd} is not
enabled), or the corresponding \texttt{sndCtr}
attribute is non-zero.
\end{itemize}
\item[2.] \texttt{mte(sysC) = 0} 
In this case some rule is enabled according to
one of the following cases.
\begin{itemize}
\item there is a message with zero delay in the net,
then the rule \texttt{rcv} is enabled (possibly preceeded by \texttt{net}) to move the message from
network input to network output;

\item there is a \texttt{w4Ack} attribute of some
endpoint with a zero delay message, then
the \texttt{ackTimeout} rule is enabled;

\item there is a \texttt{sendReqs} attribute of some
endpoint that is not empty and sending is enabled,
so the rule \texttt{devsnd} is enabled.
\end{itemize}
\item[3.] \texttt{mte(sysC) = infty}. 
In this case \texttt{sysC} is a terminal configuration, no
rules apply since the net is empty, all \texttt{w4Ack} attributes are empty, and all sendReqs are empty buy definition
of \texttt{mte}.
\end{itemize}
\end{proposition}
   
The definition of \texttt{mte} is extended to 
dialected CoAP configurations by adding 
the rule that \texttt{mte} is 0 if
any local nets are non-empty. Thus messages in
local nets must be delivered or dialected and put
in the global net before time can pass.  The
consequences are captured in the next proposition.
 
\begin{proposition}[Mte based characterization of reachable dialected CoAP configurations.]
\label{prop:mte-dialected}
As for the non-dialected case there are three cases.
\begin{itemize}
\item[1.] $\mathtt{mte(dsysC)} = \mathtt{nz:NzNat}$.
In this case the value of \texttt{mte} is determined
by the global network and the \texttt{sysC}
level attributes and only the \texttt{tick} rule (and  possibly \texttt{net}) is enabled.

\item[2.] $\mathtt{mte(dsysC)} = \mathtt{0}$.
In this case, if there is a message
some local net the either \texttt{ddevsnd} or \texttt{rcv} is enabled.  Otherwise 
either \texttt{ddevrcv} is enabled or some rule
at the \texttt{sysC}  level as shown in 
Proposition \ref{prop:mte-coap}.

\item[3.] $\mathtt{mte(dsysC)} = \mathtt{infty}$.
In this case \texttt{dsysC} is terminal.
 As for \texttt{sysC} the net is empty (global and local), \texttt{w4Ack} attributes are empty, and 
 \texttt{sendReq} attribues are empty so no rule is enabled.
\end{itemize}
\end{proposition}


  .}
  \label{apx:exe-props}

  \omitthis{
  if M is sent it will be received if not dropped
  if sv hasRspTSnt to cl tok matching aid then
  previously sv rcvd req src cl tok matching aid
  If cl hasPend sv aid then cl previously sent
  req to sv w tok matching aid
  If cl hasRspTRcd from sv mathing aid then cl previously sent req to sv w tok matching aid
  }
  

 \begin{small}
 \begin{verbatim}
 \end{verbatim}
 \end{small}
\omitthis{
\begin{proposition}[Message based characterization of reachable states]\label{prop:msg-based}

(M=m(ep0,ep1,content) in net then
 if isReq(M) then ep1 has corresponding w4 (ack or rsp) or rspRcd
 if isResp(M) then ep1 has corresponding rspSnt
      and ep0 had corresponding w4
 if isAck(M) then ep0 has matching w4Ack or a separate response
 arrived earlier and ep0 has matching rspRcd
 For every w4Ack there is the request, or a matching ack or rsp 
 in the net,  [if unreliable net modeled then the req or ack or rsp
 could have been dropped]
 if epid has rspRcd from epid0 then epid0 has corresponding rspSnt
 \end{proposition}
 
 }     

==> experiments.tex <==
\section{Summary of experiments} \label{sec:experiments}

\red{TODO: This section is an early version of
Appendix \ref{apx:coap-vulnerabilities}.  Will
be merged/revised once the dialected versions
of vulnerability scenarios are done using
the dialect transform function.}

We carried out reachability analyses for two and three
device scenarios in native CoAP configuration and in
dialected form. In each scenario the attacker has a
given goal and given capabilities and we searched for
all solutions where the attack succeeded and for all
solutions where the attack capabilities were used but
the the attack failed, i.e. the outcome was as if the
attacker were not there. The search commands are
instances of the the following patterns. The
configuration constructors \texttt{tCSA} and
\texttt{tCS3A} are defined in section
\ref{sec:coap-spec}. The configuration constructors
\texttt{testDCSA} and \texttt{tDCS3A} are defined in
section \ref{sec:coap-dialect-spec}. The goal
properties are defined in section \ref{sec:coap-spec}.

\paragraph{Two device scenario patterns for native CoAP
and dialected systems.}

 In these scenarios there is a client device with a
list of application messages \texttt{aMsgL} to send, a
server with initial resource map \texttt{rsrcs} and an
attacker with capabilities \texttt{caps}. The goal
property is \texttt{prop}. Note that the basic and
dialected patterns have the same parameters.

\noindent
\textbf{Basic CoAP search pattern.}
\begin{small}
\begin{verbatim}
    search {tCSA(aMsgL,rsrcs,caps)} =>! 
    {c:Conf ["eve" | a:Attrs caps(mtC)]} such that prop .
\end{verbatim}
\end{small}

\noindent
\textbf{Dialected CoAP search pattern.}
\begin{small}
\begin{verbatim}
    search {testDCSA(aMsgL,rsrcs,0,caps)} =>! 
    {c0:Conf ["dev{j}" | conf(c:Conf) 
             ["eve" | a:Attrs caps(mtC)]) ddattrs:Attrs]
      such that prop
\end{verbatim}
\end{small}
\noindent
In the above search patterns the exclamation point
after the arrow (\texttt{=>!}) restricts solutions
to terminal states.  The \texttt{caps(mtC)} in the
search result pattern ensures that the attacker
has exhausted its capabilities.

\paragraph{Three device scenario patterns for native CoAP and dialected systems.}

In this pattern there is one client that knows two
servers. As for the two device case, \texttt{aMsgL} is
the list of application messages for the client to
send, \texttt{rsrcs1} and \texttt{rsrcs2} are the
initial resource maps of the two servers, \texttt{caps}
is the attacker capability set, and \texttt{prop} the
desired goal.

\noindent
\textbf{Basic CoAP 3 device search pattern.}
\begin{small}
\begin{verbatim}
 search {tCS3A(aMsgL,mtR,nilAM,rsrcs1,nilAM,rsrcs2,caps)} 
    =>! {c:Conf ["eve" | a:Attrs caps(mtC)]} such that prop .
\end{verbatim}
\end{small}

\noindent
\textbf{Dialected CoAP 3 device search pattern.}
\begin{small}
\begin{verbatim}
  search {tDCS3A(aMsgL,rsrcs1,rsrcs2,caps)} 
     =>! {c0:Conf ["dev:{j}" | conf(c:Conf) ddattrs:Attrs]
          ["eve" | a:Attrs caps(mtC)]} such that prop .
\end{verbatim}
\end{small}

Table \ref{tb:experiments} sumarizes the results of the
reachability analyses. The scenario names in column
\textbf{Scenario} refer to items in the list of
scenario parameters below. Column \textbf{D?} is C for
basic CoAP instances and D for dialected versions. In
the columns \textbf{success} and \textbf{fail} an entry
\emph{n/m} means the search found \emph{n} solutions
out of \emph{m} states. For \textbf{success} the
parameter \textbf{prop} is instantiated with a property
specifying the attacker goal, and for \textbf{fail} the
parameter \textbf{prop} is instantiated with a property
specifying normal/expected execution. NS means no
solutions, in which case the normal property search was
not done (not deemed interesting).


\paragraph{Scenario parameters.}
\begin{itemize}
\item[(i)] Block response  
\begin{itemize}
\item[]\textbf{aMsgL:} \texttt{Mput ; aMgetN}
\item[]\textbf{rsrcs:} r\texttt{b("door","unlock")}
\item[]\textbf{cap:} \texttt{drop} \texttt{drop}
\item[]\textbf{j:} 0
\item[]\textbf{prop:} (success/fail)
\begin{itemize}
  \item[]
   \texttt{noRsp(c:Conf,"dev0","2.05")} /
  \item[]
   \texttt{hasGetRsp(c:Conf,"dev0","dev1","lock") }
\end{itemize}
\end{itemize}

\item[(ii)] Block request
\begin{itemize}
\item[] \textbf{aMsgL:} \texttt{aMput ; aMgetN}
\item[] \textbf{rsrcs:} \texttt{rb("door","unlock")}
\item[]\textbf{cap:} \texttt{drop} \texttt{drop}
\item[]\textbf{j:} 1
\item[]\textbf{prop}: (success/fail)
\begin{itemize}
  \item[]
  \texttt{checkRsrc(c:Conf,"dev1","door","unlock")} /
  \item[]
  \texttt{checkRsrc(c:Conf,"dev1","door","unlock")} 
\end{itemize}
\end{itemize}

\item[(iii)] Replay unlock --- reverting lock
\begin{itemize}
\item[]\textbf{aMsgL:}  \texttt{aMputU ; aMgetN ; aMput}
\item[] \textbf{rsrcs:} \texttt{rb("door","lock")}
\item[]\textbf{cap:} \texttt{replay(5/10)}
\item[]\textbf{j:} 1
\item[]\textbf{prop:} (success/fail)
\begin{itemize}
  \item[]
  \texttt{checkRsrc(c:Conf,"dev1","door","unlock")} /
  \item[]
  \texttt{checkRsrc(c:Conf,"dev1","door","unlock")} 
\end{itemize}
\end{itemize}

\item[iv] Reorder PUTs --- so door ends up unlocked
\begin{itemize}
\item[]\textbf{aMsgL:} \texttt{aMputU ; aMput}
\item[]\textbf{rsrcs:} \texttt{rb("door","unk")}
\item[]\textbf{cap:} \texttt{drop} \texttt{delay(10)}
\item[] \textbf{j:} 0
\item[]\textbf{prop:} (success/fail)
\begin{itemize}
  \item[]
  \texttt{checkRsrc(c:Conf,"dev1","door","unlock")} /
  \item[]
  \texttt{checkRsrc(c:Conf,"dev1","door","lock")} 
\end{itemize}
\end{itemize}

\item[v]  Wrong value -- client gets response of wrong device
\begin{itemize}
\item[]\textbf{aMsgL:} \texttt{aMgetN2d}
\item[]\textbf{rsrcs1:} \texttt{rb("door","lock")} 
\item[] \textbf{rsrcs2:} \texttt{rb("door","unlock")}
\item[] \textbf{caps:} \texttt{redirect("dev2","dev1")} \texttt{unredirect("dev2","dev1")}
\item[]\textbf{prop:} (success/fail)s
\begin{itemize}
  \item[]
  \texttt{hasGetRsp(c:Conf,"dev0","dev2","lock")} /
  \item[]
  \texttt{hasGetRsp(c:Conf,"dev0","dev2","unlock")}
\end{itemize}
\end{itemize}

\end{itemize}


\begin{table}[ht]
\begin{center}
  \begin{tabular}{|l|c|r|r|} %% {p{3.3cm}p{2.5cm}p{5.5cm}}
  \hline
  \textbf{Scenario}\quad &\textbf{~D?~}& \textbf{success} & \quad\textbf{fail} \\
 \hline
   (i) Block response  & C & 4/308 & 7/335 \\
                      & D & 4/2159 & 12/2370 \\
 \hline
   (ii) Block request  & C & 3/528 &  65/1015 \\
                       & D & 8/2417 & 190/7149 \\
 \hline
  (iii) Replay(5) unlock  & C & NS &  \\
                       & D & NS &  \\
 \hline
  (iii) Replay(10) unlock  & C & 2/783  & 18/787 \\
                           & D & NS &  \\
 \hline
  (iv) Reorder PUTs  & C & 54/6886 & 184/6912 \\
                     & D & 96/12393 & 664/123405\\
 \hline
  (v) Wrong value     & C & 4/33 & NS \\
                      & D & NS &     \\
 \hline
  \end{tabular}
\end{center}
\caption{Reachability results for CoAP vulnerability scenarios with and without dialect wrapping.}
\label{tb:experiments}
\end{table}


TODO -- SOME CONCLUSIONS/OBSERVATIONS

==> snd-rcv-bij.tex <==
\section{CoAP message guarantees}
\label{apx:snd-rcv-bij}

For the CoAP properties case the goal is to identify
guarantees provided by CoAP messaging running on a properly
operating unreliable transport, identify attack surfaces,
and corresponding  attack model and prove that dialecting provides adequate defense.

Properties informally:
If ep1 sends M to ep2  then
  1. M is dropped by network, or
  2. M is received by ep2 (unchanged)

If ep2 receives M from ep1 then
  previously ep1 sent this M 
  
More formally,  in terms of the CoAP specification,
let sysI  be any initial configuration 
(empty network, empty wait4s, rcds, correct link secrets ... )  
(imagine rules drop, delay added to model UDP transport)
let sysI = sys0 -r0> sys1 .... sysj -rj-> sysj+1  ... sysN terminal

Associate an event evj with each step rj as follows
rj is [rcv] evj is (rcv eid Mj) ---  tgt(Mj) == eid
rj is [devsnd] evj is (snd Mj) ---  src(Mj) == eid
rj is [ackTimout] evj is (resend  eid Mj) --- by src(Mj) of CON msg 
rj is [net]  evj is (net)
rj is [tick] evj is (tick nz)
rj is [drop] evj is (drop Mj)  --- the msg dropped
rj is [delay(k)] evj is (delay(k) Mj) the msg delayed

The semantic guarantee then is a bijection between rcv events (by tgt) and drop events (by net) and previous (re) snd (by src) events.
Probably also resend (by src) and previous drop events.
WHAT ELSE?

Let Rcv be the indices of rcv events
    Drop be the indices of drop events
    Send be the indices of devsnd events 
    ATO be the indices of acktimeout events
These sets are disjoint

More formally exists map C (for cause ) on step indices of an
execution such that

  C  : Rcv + Drop -> Send   + ATO
     such that
       C is a bijection
       C(j) < j  
       msg(C(j)) = msg(j)

Proof:
construct C as the execution unfolds.
annotate message with index of sending rule
and with index of rcving or dropping rule
Collect dropped/rcd annotated msg in a pool.
At the end they define C
   
